Power of Explanations: Towards automatic debiasing in hate speech detection

Hate speech detection is a common downstream application of natural language processing (NLP) in the real world. In spite of the increasing accuracy, current data-driven approaches could easily learn biases from the imbalanced data distributions originating from humans. The deployment of biased models could further enhance the existing social biases. But unlike handling tabular data, defining and mitigating biases in text classifiers, which deal with unstructured data, are more challenging. A popular solution for improving machine learning fairness in NLP is to conduct the debiasing process with a list of potentially discriminated words given by human annotators. In addition to suffering from the risks of overlooking the biased terms, exhaustively identifying bias with human annotators are unsustainable since discrimination is variable among different datasets and may evolve over time. To this end, we propose an automatic misuse detector (MiD) relying on an explanation method for detecting potential bias. And built upon that, an end-to-end debiasing framework with the proposed staged correction is designed for text classifiers without any external resources required.

==> bib.tex <==
@inproceedings{kennedy2020contextualizing,
  title={Contextualizing Hate Speech Classifiers with Post-hoc Explanation},
  author={Kennedy, Brendan and Jin, Xisen and Davani, Aida Mostafazadeh and Dehghani, Morteza and Ren, Xiang},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={5435--5442},
  year={2020}
}

@inproceedings{zhang2020demographics,
  title={Demographics Should Not Be the Reason of Toxicity: Mitigating Discrimination in Text Classifications with Instance Weighting},
  author={Zhang, Guanhua and Bai, Bing and Zhang, Junqi and Bai, Kun and Zhu, Conghui and Zhao, Tiejun},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={4134--4145},
  year={2020}
}

@article{yao2021refining,
  title={Refining language models with compositional explanations},
  author={Yao, Huihan and Chen, Ying and Ye, Qinyuan and Jin, Xisen and Ren, Xiang},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}

@inproceedings{zhao2018gender,
  title={Gender Bias in Coreference Resolution: Evaluation and Debiasing Methods},
  author={Zhao, Jieyu and Wang, Tianlu and Yatskar, Mark and Ordonez, Vicente and Chang, Kai-Wei},
  booktitle={Proceedings of the 2018 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  volume={2},
  year={2018}
}

@inproceedings{garg2019counterfactual,
  title={Counterfactual fairness in text classification through robustness},
  author={Garg, Sahaj and Perot, Vincent and Limtiaco, Nicole and Taly, Ankur and Chi, Ed H and Beutel, Alex},
  booktitle={Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={219--226},
  year={2019}
}

@inproceedings{kiritchenko2018examining,
  title={Examining Gender and Race Bias in Two Hundred Sentiment Analysis Systems},
  author={Kiritchenko, Svetlana and Mohammad, Saif},
  booktitle={Proceedings of the Seventh Joint Conference on Lexical and Computational Semantics},
  pages={43--53},
  year={2018}
}

@inproceedings{rudinger2018gender,
  title={Gender Bias in Coreference Resolution},
  author={Rudinger, Rachel and Naradowsky, Jason and Leonard, Brian and Van Durme, Benjamin},
  booktitle={Proceedings of NAACL-HLT},
  pages={8--14},
  year={2018}
}

@article{li2022survey,
  title={A Survey on Text Classification: From Traditional to Deep Learning},
  author={Li, Qian and Peng, Hao and Li, Jianxin and Xia, Congying and Yang, Renyu and Sun, Lichao and Yu, Philip S and He, Lifang},
  journal={ACM Transactions on Intelligent Systems and Technology (TIST)},
  volume={13},
  number={2},
  pages={1--41},
  year={2022},
  publisher={ACM New York, NY}
}

@article{muller2020ethics,
  title={Ethics of artificial intelligence and robotics},
  author={M{\"u}ller, Vincent C},
  journal={The Stanford Encyclopedia of Philosophy},
  year={2020},
  publisher={Stanford University}
}

@inproceedings{wallace2019allennlp,
  title={AllenNLP Interpret: A Framework for Explaining Predictions of NLP Models},
  author={Wallace, Eric and Tuyls, Jens and Wang, Junlin and Subramanian, Sanjay and Gardner, Matt and Singh, Sameer},
  booktitle={Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP): System Demonstrations},
  pages={7--12},
  year={2019}
}

@inproceedings{iosifidis2019fae,
  title={Fae: A fairness-aware ensemble framework},
  author={Iosifidis, Vasileios and Fetahu, Besnik and Ntoutsi, Eirini},
  booktitle={2019 IEEE International Conference on Big Data (Big Data)},
  pages={1375--1380},
  year={2019},
  organization={IEEE}
}

@inproceedings{iosifidis2019adafair,
  title={Adafair: Cumulative fairness adaptive boosting},
  author={Iosifidis, Vasileios and Ntoutsi, Eirini},
  booktitle={Proceedings of the 28th ACM International Conference on Information and Knowledge Management},
  pages={781--790},
  year={2019}
}

@article{hardt2016equality,
  title={Equality of opportunity in supervised learning},
  author={Hardt, Moritz and Price, Eric and Srebro, Nati},
  journal={Advances in neural information processing systems},
  volume={29},
  year={2016}
}

@article{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{cai2021xproax,
  title={XPROAX-Local explanations for text classification with progressive neighborhood approximation},
  author={Cai, Yi and Zimek, Arthur and Ntoutsi, Eirini},
  booktitle={2021 IEEE 8th International Conference on Data Science and Advanced Analytics (DSAA)},
  pages={1--10},
  year={2021},
  organization={IEEE}
}

@inproceedings{chen2020generating,
  title={Generating Hierarchical Explanations on Text Classification via Feature Interaction Detection},
  author={Chen, Hanjie and Zheng, Guangtao and Ji, Yangfeng},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={5578--5593},
  year={2020}
}

@inproceedings{murdoch2018beyond,
  title={Beyond Word Importance: Contextual Decomposition to Extract Interactions from LSTMs},
  author={Murdoch, W James and Liu, Peter J and Yu, Bin},
  booktitle={International Conference on Learning Representations},
  year={2018}
}

@inproceedings{jin2019towards,
  title={Towards Hierarchical Importance Attribution: Explaining Compositional Semantics for Neural Sequence Models},
  author={Jin, Xisen and Wei, Zhongyu and Du, Junyi and Xue, Xiangyang and Ren, Xiang},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@article{lundberg2017unified,
  title={A unified approach to interpreting model predictions},
  author={Lundberg, Scott M and Lee, Su-In},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@inproceedings{dixon2018measuring,
  title={Measuring and mitigating unintended bias in text classification},
  author={Dixon, Lucas and Li, John and Sorensen, Jeffrey and Thain, Nithum and Vasserman, Lucy},
  booktitle={Proceedings of the 2018 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={67--73},
  year={2018}
}

@article{schick2021self,
  title={Self-diagnosis and self-debiasing: A proposal for reducing corpus-based bias in nlp},
  author={Schick, Timo and Udupa, Sahana and Sch{\"u}tze, Hinrich},
  journal={Transactions of the Association for Computational Linguistics},
  volume={9},
  pages={1408--1424},
  year={2021},
  publisher={MIT Press}
}

@inproceedings{ribeiro2016should,
  title={" Why should i trust you?" Explaining the predictions of any classifier},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={Proceedings of the 22nd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={1135--1144},
  year={2016}
}

@inproceedings{peters2017semi,
  title={Semi-supervised sequence tagging with bidirectional language models},
  author={Peters, Matthew E and Ammar, Waleed and Bhagavatula, Chandra and Power, Russell},
  booktitle={Proceedings of the 55th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
  pages={1756--1765},
  year={2017}
}

@article{sarzynska2021detecting,
  title={Detecting formal thought disorder by deep contextualized word representations},
  author={Sarzynska-Wawer, Justyna and Wawer, Aleksander and Pawlak, Aleksandra and Szymanowska, Julia and Stefaniak, Izabela and Jarkiewicz, Michal and Okruszek, Lukasz},
  journal={Psychiatry Research},
  volume={304},
  pages={114135},
  year={2021},
  publisher={Elsevier}
}

@article{vstrumbelj2014explaining,
  title={Explaining prediction models and individual predictions with feature contributions},
  author={{\v{S}}trumbelj, Erik and Kononenko, Igor},
  journal={Knowledge and information systems},
  volume={41},
  number={3},
  pages={647--665},
  year={2014},
  publisher={Springer}
}

@article{smilkov2017smoothgrad,
  title={Smoothgrad: removing noise by adding noise},
  author={Smilkov, Daniel and Thorat, Nikhil and Kim, Been and Vi{\'e}gas, Fernanda and Wattenberg, Martin},
  journal={arXiv preprint arXiv:1706.03825},
  year={2017}
}

@inproceedings{naumann2021consequence,
  title={Consequence-aware Sequential Counterfactual Generation},
  author={Naumann, Philip and Ntoutsi, Eirini},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={682--698},
  year={2021},
  organization={Springer}
}

@inproceedings{rieger2020interpretations,
  title={Interpretations are useful: penalizing explanations to align neural networks with prior knowledge},
  author={Rieger, Laura and Singh, Chandan and Murdoch, William and Yu, Bin},
  booktitle={International conference on machine learning},
  pages={8116--8126},
  year={2020},
  organization={PMLR}
}

@inproceedings{chen2019large,
  title={How Large a Vocabulary Does Text Classification Need? A Variational Approach to Vocabulary Selection},
  author={Chen, Wenhu and Su, Yu and Shen, Yilin and Chen, Zhiyu and Yan, Xifeng and Wang, William},
  booktitle={Proceedings of NAACL-HLT},
  pages={3487--3497},
  year={2019}
}

@article{zhuang2022randomness,
  title={Randomness in neural network training: Characterizing the impact of tooling},
  author={Zhuang, Donglin and Zhang, Xingyao and Song, Shuaiwen and Hooker, Sara},
  journal={Proceedings of Machine Learning and Systems},
  volume={4},
  year={2022}
}

@article{kennedy2018gab,
  title={The Gab Hate Corpus: A collection of 27k posts annotated for hate speech},
  author={Kennedy, Brendan and Atari, Mohammad and Davani, Aida Mostafazadeh and Yeh, Leigh and Omrani, Ali and Kim, Yehsong and Coombs, Kris and Havaldar, Shreya and Portillo-Wightman, Gwenyth and Gonzalez, Elaine and others},
  publisher={PsyArXiv}
}

@article{anthony2016inside,
  title={Inside the hate-filled echo chamber of racism and conspiracy theories},
  author={Anthony, Andrew},
  journal={The guardian},
  volume={18},
  year={2016}
}

@inproceedings{kenton2019bert,
  title={BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding},
  author={Kenton, Jacob Devlin Ming-Wei Chang and Toutanova, Lee Kristina},
  booktitle={Proceedings of NAACL-HLT},
  pages={4171--4186},
  year={2019}
}

@inproceedings{zhang2021explain,
  title={Explain and predict, and then predict again},
  author={Zhang, Zijian and Rudra, Koustav and Anand, Avishek},
  booktitle={Proceedings of the 14th ACM International Conference on Web Search and Data Mining},
  pages={418--426},
  year={2021}
}

@inproceedings{wolf2020transformers,
  title={Transformers: State-of-the-art natural language processing},
  author={Wolf, Thomas and Debut, Lysandre and Sanh, Victor and Chaumond, Julien and Delangue, Clement and Moi, Anthony and Cistac, Pierric and Rault, Tim and Louf, R{\'e}mi and Funtowicz, Morgan and others},
  booktitle={Proceedings of the 2020 conference on empirical methods in natural language processing: system demonstrations},
  pages={38--45},
  year={2020}
}

@article{bhardwaj2021investigating,
  title={Investigating gender bias in BERT},
  author={Bhardwaj, Rishabh and Majumder, Navonil and Poria, Soujanya},
  journal={Cognitive Computation},
  volume={13},
  number={4},
  pages={1008--1018},
  year={2021},
  publisher={Springer}
}

@article{ahn2021mitigating,
  title={Mitigating language-dependent ethnic bias in BERT},
  author={Ahn, Jaimeen and Oh, Alice},
  journal={arXiv preprint arXiv:2109.05704},
  year={2021}
}
